Le cristal de Dieudonn\'e des sch\'emas en $\mathbb{F}$-vectoriels

In this paper we describe the Dieudonn\'e crystal of a finite locally free group scheme with a vector action of a finite field $\mathbb{F}$. These $\mathbb{F}$-vector schemes appear when we consider torsion points of $p$-divisible modules. A particular class of $\mathbb{F}$-vector schemes has been classified by Raynaud in [Ray74], which allows us to determine the structure of torsion points of $p$-divisible modules, under certain conditions on the Lie algebra.

==> macmacro.tex <==
\usepackage{amsthm,amsfonts,amssymb,amsmath,amsxtra}
\usepackage[all]{xy}
% force xy arrow tips in computer modern font:
\SelectTips{cm}{}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{verbatim}
% \usepackage{pdfsync}
% \usepackage{showkeys}

\usepackage[margin=1.25in]{geometry}
\usepackage{mathrsfs}

\usepackage[french]{babel}
\usepackage[T1]{fontenc} %accents
% for smart spacing after certain commands:
\RequirePackage{xspace}
% for programming features:
\RequirePackage{etoolbox}
% for text environments which are automatically the natural width of the text they contain:
\RequirePackage{varwidth}
% for easy margin adjustment in enumerate and itemize environments:
\RequirePackage{enumitem}
% for good placement of super/subscripts to the left of symbols:
\RequirePackage{tensor}
% for various extensions of amsmath:
\RequirePackage{mathtools}
% allow tables to (if needed) split over multiple pages:
\RequirePackage{longtable}
% allow cells spanning multiple rows in tables:
\RequirePackage{multirow}
% allow nice line breaks inside cells (with \makecell{}):
\RequirePackage{makecell}
% for big integral signs:
\RequirePackage{bigints}
% for upward diagonal dots:
\RequirePackage{mathdots}

\usepackage{stmaryrd}

\usepackage{hyperref} %[backref=page]




% put sections only (as opposed to subsections) in the table of contents
\setcounter{tocdepth}{1}


\newcommand{\sA}{\ensuremath{\mathscr{A}}\xspace}
\newcommand{\sB}{\ensuremath{\mathscr{B}}\xspace}
\newcommand{\sC}{\ensuremath{\mathscr{C}}\xspace}
\newcommand{\sD}{\ensuremath{\mathscr{D}}\xspace}
\newcommand{\sE}{\ensuremath{\mathscr{E}}\xspace}
\newcommand{\sF}{\ensuremath{\mathscr{F}}\xspace}
\newcommand{\sG}{\ensuremath{\mathscr{G}}\xspace}
\newcommand{\sH}{\ensuremath{\mathscr{H}}\xspace}
\newcommand{\sI}{\ensuremath{\mathscr{I}}\xspace}
\newcommand{\sJ}{\ensuremath{\mathscr{J}}\xspace}
\newcommand{\sK}{\ensuremath{\mathscr{K}}\xspace}
\newcommand{\sL}{\ensuremath{\mathscr{L}}\xspace}
\newcommand{\sM}{\ensuremath{\mathscr{M}}\xspace}
\newcommand{\sN}{\ensuremath{\mathscr{N}}\xspace}
\newcommand{\sO}{\ensuremath{\mathscr{O}}\xspace}
\newcommand{\sP}{\ensuremath{\mathscr{P}}\xspace}
\newcommand{\sQ}{\ensuremath{\mathscr{Q}}\xspace}
\newcommand{\sR}{\ensuremath{\mathscr{R}}\xspace}
\newcommand{\sS}{\ensuremath{\mathscr{S}}\xspace}
\newcommand{\sT}{\ensuremath{\mathscr{T}}\xspace}
\newcommand{\sU}{\ensuremath{\mathscr{U}}\xspace}
\newcommand{\sV}{\ensuremath{\mathscr{V}}\xspace}
\newcommand{\sW}{\ensuremath{\mathscr{W}}\xspace}
\newcommand{\sX}{\ensuremath{\mathscr{X}}\xspace}
\newcommand{\sY}{\ensuremath{\mathscr{Y}}\xspace}
\newcommand{\sZ}{\ensuremath{\mathscr{Z}}\xspace}


\newcommand{\fka}{\ensuremath{\mathfrak{a}}\xspace}
\newcommand{\fkb}{\ensuremath{\mathfrak{b}}\xspace}
\newcommand{\fkc}{\ensuremath{\mathfrak{c}}\xspace}
\newcommand{\fkd}{\ensuremath{\mathfrak{d}}\xspace}
\newcommand{\fke}{\ensuremath{\mathfrak{e}}\xspace}
\newcommand{\fkf}{\ensuremath{\mathfrak{f}}\xspace}
\newcommand{\fkg}{\ensuremath{\mathfrak{g}}\xspace}
\newcommand{\fkh}{\ensuremath{\mathfrak{h}}\xspace}
\newcommand{\fki}{\ensuremath{\mathfrak{i}}\xspace}
\newcommand{\fkj}{\ensuremath{\mathfrak{j}}\xspace}
\newcommand{\fkk}{\ensuremath{\mathfrak{k}}\xspace}
\newcommand{\fkl}{\ensuremath{\mathfrak{l}}\xspace}
\newcommand{\fkm}{\ensuremath{\mathfrak{m}}\xspace}
\newcommand{\fkn}{\ensuremath{\mathfrak{n}}\xspace}
\newcommand{\fko}{\ensuremath{\mathfrak{o}}\xspace}
\newcommand{\fkp}{\ensuremath{\mathfrak{p}}\xspace}
\newcommand{\fkq}{\ensuremath{\mathfrak{q}}\xspace}
\newcommand{\fkr}{\ensuremath{\mathfrak{r}}\xspace}
\newcommand{\fks}{\ensuremath{\mathfrak{s}}\xspace}
\newcommand{\fkt}{\ensuremath{\mathfrak{t}}\xspace}
\newcommand{\fku}{\ensuremath{\mathfrak{u}}\xspace}
\newcommand{\fkv}{\ensuremath{\mathfrak{v}}\xspace}
\newcommand{\fkw}{\ensuremath{\mathfrak{w}}\xspace}
\newcommand{\fkx}{\ensuremath{\mathfrak{x}}\xspace}
\newcommand{\fky}{\ensuremath{\mathfrak{y}}\xspace}
\newcommand{\fkz}{\ensuremath{\mathfrak{z}}\xspace}


\newcommand{\fkA}{\ensuremath{\mathfrak{A}}\xspace}
\newcommand{\fkB}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\fkC}{\ensuremath{\mathfrak{C}}\xspace}
\newcommand{\fkD}{\ensuremath{\mathfrak{D}}\xspace}
\newcommand{\fkE}{\ensuremath{\mathfrak{E}}\xspace}
\newcommand{\fkF}{\ensuremath{\mathfrak{F}}\xspace}
\newcommand{\fkG}{\ensuremath{\mathfrak{G}}\xspace}
\newcommand{\fkH}{\ensuremath{\mathfrak{H}}\xspace}
\newcommand{\fkI}{\ensuremath{\mathfrak{I}}\xspace}
\newcommand{\fkJ}{\ensuremath{\mathfrak{J}}\xspace}
\newcommand{\fkK}{\ensuremath{\mathfrak{K}}\xspace}
\newcommand{\fkL}{\ensuremath{\mathfrak{L}}\xspace}
\newcommand{\fkM}{\ensuremath{\mathfrak{M}}\xspace}
\newcommand{\fkN}{\ensuremath{\mathfrak{N}}\xspace}
\newcommand{\fkO}{\ensuremath{\mathfrak{O}}\xspace}
\newcommand{\fkP}{\ensuremath{\mathfrak{P}}\xspace}
\newcommand{\fkQ}{\ensuremath{\mathfrak{Q}}\xspace}
\newcommand{\fkR}{\ensuremath{\mathfrak{R}}\xspace}
\newcommand{\fkS}{\ensuremath{\mathfrak{S}}\xspace}
\newcommand{\fkT}{\ensuremath{\mathfrak{T}}\xspace}
\newcommand{\fkU}{\ensuremath{\mathfrak{U}}\xspace}
\newcommand{\fkV}{\ensuremath{\mathfrak{V}}\xspace}
\newcommand{\fkW}{\ensuremath{\mathfrak{W}}\xspace}
\newcommand{\fkX}{\ensuremath{\mathfrak{X}}\xspace}
\newcommand{\fkY}{\ensuremath{\mathfrak{Y}}\xspace}
\newcommand{\fkZ}{\ensuremath{\mathfrak{Z}}\xspace}


\newcommand{\BA}{\ensuremath{\mathbb{A}}\xspace}
\newcommand{\BB}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\BC}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\BD}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\BE}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\BF}{\ensuremath{\mathbb{F}}\xspace}
\newcommand{\BG}{\ensuremath{\mathbb{G}}\xspace}
\newcommand{\BH}{\ensuremath{\mathbb{H}}\xspace}
\newcommand{\BI}{\ensuremath{\mathbb{I}}\xspace}
\newcommand{\BJ}{\ensuremath{\mathbb{J}}\xspace}
\newcommand{\BK}{\ensuremath{\mathbb{K}}\xspace}
\newcommand{\BL}{\ensuremath{\mathbb{L}}\xspace}
\newcommand{\BM}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\BN}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\BO}{\ensuremath{\mathbb{O}}\xspace}
\newcommand{\BP}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\BQ}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\BR}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\BS}{\ensuremath{\mathbb{S}}\xspace}
\newcommand{\BT}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\BU}{\ensuremath{\mathbb{U}}\xspace}
\newcommand{\BV}{\ensuremath{\mathbb{V}}\xspace}
\newcommand{\BW}{\ensuremath{\mathbb{W}}\xspace}
\newcommand{\BX}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\BY}{\ensuremath{\mathbb{Y}}\xspace}
\newcommand{\BZ}{\ensuremath{\mathbb{Z}}\xspace}


\newcommand{\bA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\bB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\bC}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\bD}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\bE}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\bF}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\bG}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\bH}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\bI}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\bJ}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\bK}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\bL}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\bM}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\bN}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\bO}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\bP}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\bQ}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\bR}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\bS}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\bT}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\bU}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\bV}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\bW}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\bX}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}\xspace}


\newcommand{\ba}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\bb}{\ensuremath{\mathbf{b}}\xspace}
\newcommand{\bc}{\ensuremath{\mathbf{c}}\xspace}
\newcommand{\bd}{\ensuremath{\mathbf{d}}\xspace}
\newcommand{\be}{\ensuremath{\mathbf{e}}\xspace}
\newcommand{\bbf}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\bg}{\ensuremath{\mathbf{g}}\xspace}
\newcommand{\bh}{\ensuremath{\mathbf{h}}\xspace}
\newcommand{\bi}{\ensuremath{\mathbf{i}}\xspace}
\newcommand{\bj}{\ensuremath{\mathbf{j}}\xspace}
\newcommand{\bk}{\ensuremath{\mathbf{k}}\xspace}
\newcommand{\bl}{\ensuremath{\mathbf{l}}\xspace}
\newcommand{\bm}{\ensuremath{\mathbf{m}}\xspace}
\newcommand{\bn}{\ensuremath{\mathbf{n}}\xspace}
\newcommand{\bo}{\ensuremath{\mathbf{o}}\xspace}
\newcommand{\bp}{\ensuremath{\mathbf{p}}\xspace}
\newcommand{\bq}{\ensuremath{\mathbf{q}}\xspace}
\newcommand{\br}{\ensuremath{\mathbf{r}}\xspace}
\newcommand{\bbs}{\ensuremath{\mathbf{s}}\xspace}
\newcommand{\bt}{\ensuremath{\mathbf{t}}\xspace}
\newcommand{\bu}{\ensuremath{\mathbf{u}}\xspace}
\newcommand{\bv}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\bw}{\ensuremath{\mathbf{w}}\xspace}
\newcommand{\bx}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\by}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\bz}{\ensuremath{\mathbf{z}}\xspace}


\newcommand{\CA}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\CB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\CC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\CD}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\CE}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\CF}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\CG}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\CH}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\CI}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\CJ}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\CK}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\CL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\CM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\CN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\CO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\CP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\CQ}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\CR}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\CS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\CT}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\CU}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\CV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\CW}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\CX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\CY}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\CZ}{\ensuremath{\mathcal{Z}}\xspace}


\newcommand{\RA}{\ensuremath{\mathrm{A}}\xspace}
\newcommand{\RB}{\ensuremath{\mathrm{B}}\xspace}
\newcommand{\RC}{\ensuremath{\mathrm{C}}\xspace}
\newcommand{\RD}{\ensuremath{\mathrm{D}}\xspace}
\newcommand{\RE}{\ensuremath{\mathrm{E}}\xspace}
\newcommand{\RF}{\ensuremath{\mathrm{F}}\xspace}
\newcommand{\RG}{\ensuremath{\mathrm{G}}\xspace}
\newcommand{\RH}{\ensuremath{\mathrm{H}}\xspace}
\newcommand{\RI}{\ensuremath{\mathrm{I}}\xspace}
\newcommand{\RJ}{\ensuremath{\mathrm{J}}\xspace}
\newcommand{\RK}{\ensuremath{\mathrm{K}}\xspace}
\newcommand{\RL}{\ensuremath{\mathrm{L}}\xspace}
\newcommand{\RM}{\ensuremath{\mathrm{M}}\xspace}
\newcommand{\RN}{\ensuremath{\mathrm{N}}\xspace}
\newcommand{\RO}{\ensuremath{\mathrm{O}}\xspace}
\newcommand{\RP}{\ensuremath{\mathrm{P}}\xspace}
\newcommand{\RQ}{\ensuremath{\mathrm{Q}}\xspace}
\newcommand{\RR}{\ensuremath{\mathrm{R}}\xspace}
\newcommand{\RS}{\ensuremath{\mathrm{S}}\xspace}
\newcommand{\RT}{\ensuremath{\mathrm{T}}\xspace}
\newcommand{\RU}{\ensuremath{\mathrm{U}}\xspace}
\newcommand{\RV}{\ensuremath{\mathrm{V}}\xspace}
\newcommand{\RW}{\ensuremath{\mathrm{W}}\xspace}
\newcommand{\RX}{\ensuremath{\mathrm{X}}\xspace}
\newcommand{\RY}{\ensuremath{\mathrm{Y}}\xspace}
\newcommand{\RZ}{\ensuremath{\mathrm{Z}}\xspace}


\newcommand{\uF}{\underline{F}}
\newcommand{\uV}{\underline{V}}





\newcommand{\heart}{{\heartsuit}}
\newcommand{\club}{{\clubsuit}}
\newcommand{\nat}{{\natural}}
\newcommand{\shp}{{\sharp}}
%\newcommand{\flat}{{\flat}}
\newcommand{\diam}{{\Diamond}}
\newcommand{\spade}{{\spadesuit}}





\DeclareMathOperator{\W}{W}
\newcommand{\CoW}{\mathrm{CW}}
\newcommand{\ab}{\mathrm{ab}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\alb}{\mathrm{alb}}
\newcommand{\AT}{\mathrm{AT}}
\DeclareMathOperator{\Cha}{Ch}
\DeclareMathOperator{\cha}{\mathfrak{ch}}
\DeclareMathOperator{\Aut}{Aut}

\newcommand{\Br}{{\mathrm{Br}}}

\newcommand{\cay}{\ensuremath{\operatorname{\fkc_\xi}}\xspace}
\newcommand{\Ch}{{\mathrm{Ch}}}
\DeclareMathOperator{\charac}{char}
\DeclareMathOperator{\Coker}{Coker}
\newcommand{\cod}{{\mathrm{cod}}}
\DeclareMathOperator{\colspan}{colspan}
\newcommand{\cont}{{\mathrm{cont}}}
\newcommand{\cl}{{\mathrm{cl}}}
\newcommand{\Cl}{{\mathrm{Cl}}}
\newcommand{\cm}{{\mathrm {cm}}}
\newcommand{\corr}{\mathrm{corr}}

\newcommand{\del}{\operatorname{\partial Orb}}
\newcommand{\delJ}{\partial J}
\DeclareMathOperator{\diag}{diag}
\newcommand{\disc}{{\mathrm{disc}}}
\DeclareMathOperator{\dist}{dist}
\newcommand{\Div}{{\mathrm{Div}}}
\renewcommand{\div}{{\mathrm{div}}}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\Dr}{\mathrm{Dr}}

\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\sEnd}{\sE nd}
\DeclareMathOperator{\sExt}{\sE xt}

\newcommand{\Fil}{\ensuremath{\mathrm{Fil}}\xspace}
\newcommand{\fin}{\mathrm{fin}}
\DeclareMathOperator{\Frob}{Frob}
\newcommand{\Mdr}[1]{{\mathscr{M}^{#1}_{\rm{Dr}}}}
\newcommand{\Mray}[1]{\mathscr{M}_{#1\rm{-Ray}}}
\newcommand*{\isoarrow}[1]{\arrow[#1,"\rotatebox{90}{\(\sim\)}"]}


\DeclareMathOperator{\Gal}{Gal}
\newcommand{\gen}{\mathrm{generic}}
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\gl}{\frak{gl}}
\newcommand{\GO}{\mathrm{GO}}
\DeclareMathOperator{\Gr}{Gr}
\newcommand{\gr}{\mathrm{gr}}
\newcommand{\GS}{\mathrm{GS}}
\newcommand{\GSpin}{\mathrm{GSpin}}
\newcommand{\GU}{\mathrm{GU}}
\newcommand{\BrTi}{\mathcal{BT}}

\newcommand{\hg}{{\mathrm{hg}}}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\sHom}{\mathscr{H}om}
\DeclareMathOperator{\Norm}{N}
\DeclareMathOperator{\Agen}{\mathbf{-Gen}}
\DeclareMathOperator{\Sch}{\mathbf{Sch}}
\DeclareMathOperator{\Vect}{\mathbf{Vect}}
\DeclareMathOperator{\Nilp}{\mathbf{Nilp}}
\DeclareMathOperator{\Fin}{\mathbf{Fin}}
\DeclareMathOperator{\proFin}{\mathbf{pro-Fin}}
\DeclareMathOperator{\Set}{\mathbf{Sets}}
\DeclareMathOperator{\okalg}{\mathbf{Alg}}
\DeclareMathOperator{\oktopalg}{\mathbf{AlgAd}}
\DeclareMathOperator{\ann}{\mathbf{Ann}}
\DeclareMathOperator{\grpab}{\mathbf{GrpAb}}
\DeclareMathOperator{\okmod}{\mathbf{Mod}}
\DeclareMathOperator{\oktopmod}{\mathbf{TopMod}}
\DeclareMathOperator{\Schfor}{\mathbf{SchFor}}
\DeclareMathOperator{\Rig}{\mathbf{Rig}}
\DeclareMathOperator{\ens}{\mathbf{Ens}}


\newcommand{\id}{\ensuremath{\mathrm{id}}\xspace}
\let\Im\relax
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Im}{Im}
\renewcommand{\i}{^{-1}}
\newcommand{\Ind}{{\mathrm{Ind}}}
\newcommand{\inj}{\hookrightarrow}
\DeclareMathOperator{\Int}{\ensuremath{\mathrm{Int}}\xspace}
\newcommand{\inv}{{\mathrm{inv}}}
\DeclareMathOperator{\Isom}{Isom}


\DeclareMathOperator{\Jac}{Jac}

 \DeclareMathOperator{\coker}{coker}

\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\Lie}{Lie}
\newcommand{\lInt}{\ensuremath{\text{$\ell$-}\mathrm{Int}}\xspace}
\newcommand{\loc}{\ensuremath{\mathrm{loc}}\xspace}

\newcommand{\Mp}{{\mathrm{Mp}}}

\newcommand{\naive}{\ensuremath{\mathrm{naive}}\xspace}
\newcommand{\new}{{\mathrm{new}}}
%\newcommand{\Nilp}{\ensuremath{\mathtt{Nilp}}\xspace}
\newcommand{\ngen}{\mathrm{non\text{-}generic}}
\DeclareMathOperator{\Nm}{Nm}
\DeclareMathOperator{\NS}{NS}

\newcommand{\OGr}{\mathrm{OGr}}
\DeclareMathOperator{\Orb}{Orb}
\DeclareMathOperator{\ord}{ord}

\DeclareMathOperator{\proj}{proj}

\DeclareMathOperator{\rang}{rang}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Ros}{Ros}

\newcommand{\PGL}{{\mathrm{PGL}}}
\DeclareMathOperator{\Pic}{Pic}

\newcommand{\rc}{\ensuremath{\mathrm{rc}}\xspace}
\renewcommand{\Re}{{\mathrm{Re}}}
\newcommand{\red}{\ensuremath{\mathrm{red}}\xspace}
\newcommand{\reg}{{\mathrm{reg}}}
\DeclareMathOperator{\Res}{Res}
\newcommand{\rs}{\ensuremath{\mathrm{rs}}\xspace}

\newcommand{\Sel}{{\mathrm{Sel}}}
\newcommand{\Sh}{\mathrm{Sh}}
%\newcommand{\Sha}{{\underline{\mathrm{|||}}}}
%\newcommand{\Sha}{{\hbox{\cyr Sh}}
\newcommand{\Sim}{{\mathrm{Sim}}}
\newcommand{\SL}{{\mathrm{SL}}}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spf}{Spf}
\DeclareMathOperator{\Spm}{Spm}
\DeclareMathOperator{\Proj}{Proj}
\newcommand{\spin}{\ensuremath{\mathrm{spin}}\xspace}
\newcommand{\SO}{{\mathrm{SO}}}
\newcommand{\Sp}{{\mathrm{Sp}}}
\newcommand{\spl}{\mathrm{split}}
\newcommand{\SU}{{\mathrm{SU}}}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\CRIS}{CRIS}

\DeclareMathOperator{\tr}{tr}
\newcommand{\triv}{\mathrm{triv}}

\newcommand{\U}{\mathrm{U}}
\DeclareMathOperator{\uAut}{\underline{Aut}}
\newcommand{\ur}{{\mathrm{ur}}}

\DeclareMathOperator{\vol}{vol}

\DeclareMathOperator{\WT}{WT}
\newcommand{\wtHG}{\ensuremath{{\widetilde{{H\! G}}}}\xspace}


\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\pp}{\frac{\partial\ov\partial}{\pi i}}
\newcommand{\pair}[1]{\langle {#1} \rangle}
\newcommand{\wpair}[1]{\left\{{#1}\right\}}
\newcommand{\intn}[1]{\left( {#1} \right)}
\newcommand{\norm}[1]{\|{#1}\|}
\newcommand{\sfrac}[2]{\left( \frac {#1}{#2}\right)}
\newcommand{\ds}{\displaystyle}
\newcommand{\ov}{\overline}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\lra}{\longrightarrow}
\newcommand{\imp}{\Longrightarrow}
\newcommand{\lto}{\longmapsto}
\newcommand{\bs}{\backslash}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lv}{\lvert}
\newcommand{\rv}{\rvert}
\newcommand{\sidewedge}[1]{\sideset{}{#1}\bigwedge}

%restriction 

\def\restriction#1#2{\mathchoice
              {\setbox1\hbox{${\displaystyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\textstyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptscriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}}
\def\restrictionaux#1#2{{#1\,\smash{\vrule height .8\ht1 depth .85\dp1}}_{\,#2}} 


\newcommand{\ep}{\varepsilon}

%%% some additional macros


\newcommand{\nass}{\noalign{\smallskip}}
\newcommand{\htt}{h}
\newcommand{\cutter}{\medskip\medskip \hrule \medskip\medskip}



% Equation  \AMSname
% Theorem   \theoremname


% Theorem environments.
%
\newtheorem{theorem}{Théorème}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemme}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{`conjecture'}[theorem]{``Conjecture''}
\newtheorem{corollary}[theorem]{Corollaire}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Définition}
\newtheorem{example}[theorem]{Exemple}
\newtheorem{exercise}[theorem]{Exercice}
\newtheorem{situation}[theorem]{Situation}
\newtheorem{remark}[theorem]{Remarque}
\newtheorem{remarks}[theorem]{Remarque}
\newtheorem{question}[theorem]{Question}

\newenvironment{altenumerate}
   {\begin{list}
      {(\theenumi) }
      {\usecounter{enumi}
       \setlength{\labelwidth}{0pt}
       \setlength{\labelsep}{0pt}
       \setlength{\leftmargin}{0pt}
       \setlength{\itemsep}{\the\smallskipamount}
       \renewcommand{\theenumi}{\roman{enumi}}
      }}
   {\end{list}}
% the following is a "level 2" altenumerate
\newenvironment{altenumerate2}
   {\begin{list}
      {\textup{(\theenumii)} }
      {\usecounter{enumii}
       \setlength{\labelwidth}{0pt}
       \setlength{\labelsep}{0pt}
       \setlength{\leftmargin}{2em}
       \setlength{\itemsep}{\the\smallskipamount}
       \renewcommand{\theenumii}{\alph{enumii}}
      }}
   {\end{list}}

\newenvironment{altitemize}
   {\begin{list}
      {$\bullet$}
      {\setlength{\labelwidth}{0pt}
	   \setlength{\itemindent}{5pt}
       \setlength{\labelsep}{5pt}
       \setlength{\leftmargin}{0pt}
       \setlength{\itemsep}{\the\smallskipamount}
      }}
   {\end{list}}




\numberwithin{equation}{section}
\numberwithin{theorem}{section}



%%%% macros added by Brian
%%%% many of these require the etoolbox package, which should be loaded above

\newcommand{\aform}{\ensuremath{\langle\text{~,~}\rangle}\xspace}
\newcommand{\sform}{\ensuremath{(\text{~,~})}\xspace}

\newcounter{filler}
\newcounter{ATtype}

% gets rid of indentation in itemize and enumerate enivronments, and adds
% a small space between list items:
\setitemize[0]{leftmargin=*,itemsep=\the\smallskipamount}
\setenumerate[0]{leftmargin=*,itemsep=\the\smallskipamount}

% basic right arrow, short in inlines and long in displays
\renewcommand{\to}{%
   \ifbool{@display}{\longrightarrow}{\rightarrow}%
   }
% redefine \mapsto to be short in inlines and long in displays
\let\shortmapsto\mapsto
\renewcommand{\mapsto}{%
   \ifbool{@display}{\longmapsto}{\shortmapsto}%
   }
% stretchable labeled right (2nd is xy-style) & left arrows, well-behaved inline or displayed
\newlength{\olen}
\newlength{\ulen}
\newlength{\xlen}
\newcommand{\xra}[2][]{%
   \ifbool{@display}%
      {\settowidth{\olen}{$\overset{#2}{\longrightarrow}$}%
       \settowidth{\ulen}{$\underset{#1}{\longrightarrow}$}%
       \settowidth{\xlen}{$\xrightarrow[#1]{#2}$}%
       \ifdimgreater{\olen}{\xlen}%
          {\underset{#1}{\overset{#2}{\longrightarrow}}}%
          {\ifdimgreater{\ulen}{\xlen}%
             {\underset{#1}{\overset{#2}{\longrightarrow}}}
             {\xrightarrow[#1]{#2}}}}%
      {\xrightarrow[#1]{#2}}
   }
\makeatother
\newcommand{\xyra}[2][]{%
   \settowidth{\xlen}{$\xrightarrow[#1]{#2}$}%
   \ifbool{@display}%
      {\settowidth{\olen}{$\overset{#2}{\longrightarrow}$}%
       \settowidth{\ulen}{$\underset{#1}{\longrightarrow}$}%
       \ifdimgreater{\olen}{\xlen}%
          {\mathrel{\xymatrix@M=.12ex@C=3.2ex{\ar[r]^-{#2}_-{#1} &}}}%
          {\ifdimgreater{\ulen}{\xlen}%
             {\mathrel{\xymatrix@M=.12ex@C=3.2ex{\ar[r]^-{#2}_-{#1} &}}}
             {\mathrel{\xymatrix@M=.12ex@C=\the\xlen{\ar[r]^-{#2}_-{#1} &}}}}}%
      {\mathrel{\xymatrix@M=.12ex@C=\the\xlen{\ar[r]^-{#2}_-{#1} &}}}%
   }
\makeatletter
\newcommand{\xla}[2][]{%
   \ifbool{@display}%
      {\settowidth{\olen}{$\overset{#2}{\longleftarrow}$}%
       \settowidth{\ulen}{$\underset{#1}{\longleftarrow}$}%
       \settowidth{\xlen}{$\xleftarrow[#1]{#2}$}%
       \ifdimgreater{\olen}{\xlen}%
          {\underset{#1}{\overset{#2}{\longleftarrow}}}%
          {\ifdimgreater{\ulen}{\xlen}%
             {\underset{#1}{\overset{#2}{\longleftarrow}}}
             {\xleftarrow[#1]{#2}}}}%
      {\xleftarrow[#1]{#2}}
   }
% isomorphism arrow, short in inlines and long in displays
%\newcommand{\isoarrow}{%
%   \ifbool{@display}{\overset{\sim}{\longrightarrow}}{\xrightarrow\sim}%
   %}
% left-right arrow, short inline and long in diplays
\renewcommand{\lra}{%
   \ifbool{@display}{\longleftrightarrow}{\leftrightarrow}%
   }
% tilde for use under arrows (e.g. \xra) to designate isomorphisms
\newcommand{\undertilde}{\raisebox{0.4ex}{\smash[t]{$\scriptstyle\sim$}}}  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
